Exponential Family Attention

The self-attention mechanism is the backbone of the transformer neural network underlying most large language models. It can capture complex word patterns and long-range dependencies in natural language. This paper introduces exponential family attention (EFA), a probabilistic generative model that extends self-attention to handle high-dimensional sequence, spatial, or spatial-temporal data of mixed data types, including both discrete and continuous observations. The key idea of EFA is to model each observation conditional on all other existing observations, called the context, whose relevance is learned in a data-driven way via an attention-based latent factor model. In particular, unlike static latent embeddings, EFA uses the self-attention mechanism to capture dynamic interactions in the context, where the relevance of each context observations depends on other observations. We establish an identifiability result and provide a generalization guarantee on excess loss for EFA. Across real-world and synthetic data sets -- including U.S. city temperatures, Instacart shopping baskets, and MovieLens ratings -- we find that EFA consistently outperforms existing models in capturing complex latent structures and reconstructing held-out data.

==> efa.tex <==
% !TeX root = ./main.tex

\section{Exponential Family Attention}
\label{sec:efattn}
\textbf{The limitations of EFE.} Recall that in Exponential Family Embeddings (EFE), each data point is modeled based on its context, i.e., $$x_i \mid x_{c_i} \sim \textrm{ExpFam}(\eta_i(x_{c_i}), t(x_i)),$$ where $$\eta_i(x_{c_i}) := f_i \left(\rho[i]^\top \sum_{j \in c_i} \alpha[j] x_j \right).$$ However, this formulation has three notable limitations related to \textit{linearity}, \textit{order invariance}, and \textit{context definition}.

First, the expression inside $f_i$ is linear, as it assumes an additive effect from each element in the context. This limits the expressivity of the model, making it less capable of capturing non-linear relationships within the data. For example, in word embeddings, the relationship between words in a sentence might depend on their interactions rather than simply their additive contributions. In the movie ratings example (Example \ref{ex:ratings}), the combined impact of the ratings of two different movies rated by the same user on another movie's rating may involve interactions that a simple summation cannot adequately capture.

Second, EFE is inherently order invariant. In the case where $\alpha[j] = \alpha$, as in Continuous Bag of Words (CBOW), the order of elements (e.g., words) in the context does not affect the conditional distribution $x_i \mid x_{c_i}$. Even when $\alpha[j]$ varies across $j$, as in the movie ratings example (Example \ref{ex:ratings}), the order in which the elements of the context are observed does not influence $x_i \mid x_{c_i}$. Unfortunately, this assumption is unlikely to hold in many real-world settings. For example, the order in which a user rates movies may reflect temporal or sequential preferences that are relevant to predicting future ratings.

Third, it can be challenging to appropriately define the context. In CBOW, the window size around each target word needs to be carefully chosen, as it directly affects the model's performance. A window that is too small may miss critical contextual information, whereas one that is too large may include irrelevant information. Similarly, in the Gaussian observations example (Example \ref{ex:gauss}), defining the context involves determining what ``closeness" means and choosing the appropriate value of $k$.

\noindent
\textbf{From EFE to EFA.} To simultaneously address these limitations, we propose \textit{Exponential Family Attention} (EFA), whose goal is to improve the flexibility and expressiveness of EFE by incorporating the self-attention mechanism \citep{vaswani2017attention} into the model. This approach is motivated by how Bidirectional Encoder Representations from Transformers (BERT) \citep{devlin2019bert}, a bidirectional language model based on self-attention, extends the CBOW model.

\noindent
\textbf{Organization of this section.} The remainder of this section is structured as follows. Section \ref{sec:bert} provides an overview of the BERT architecture and its masked language model (MLM) training objective. Section \ref{sec:bert-cbow} demonstrates that BERT can be understood as a generalization of CBOW. Section \ref{sec: efa-efe} presents EFA as a broader form of EFE and discusses its benefits over EFE.

\subsection{BERT and the masked language model objective}
\label{sec:bert}
BERT \citep{devlin2019bert} is an attention-based model for language understanding that employs a bidirectional approach, i.e., considering both the left and right context of each word. It consists of two main training objectives: \textit{masked language model} (MLM) (predicting randomly masked tokens within a sentence) and \textit{next sentence prediction} (determining whether one sentence logically follows another). For the purposes of our discussion, we focus on a simplified version of BERT that only incorporates the MLM objective, where a single word in a sentence is randomly masked at a time.

\noindent
\textbf{Formalization.} Suppose we are given a sentence $x = x_{1:I}$, where $I$ denotes the sentence length. Also, let the vocabulary size be $D$ (thus $x_i \in [D]$ for each $i \in [I]$). In order to predict $x_i$, i.e., the $i$-th token of the sentence, the model performs the following steps:
\begin{enumerate}[leftmargin=0.6cm]
    \item Replace $x_i$ with the \texttt{[MASK]} token; the sentence is now $(x_1, \dots, x_{i-1}, \texttt{[MASK]}, x_{i+1}, \dots, x_I)$.
    \item Introduce a \textit{context embedding} $\beta_\ell \in \mathbb{R}^K$ for each token $\ell \in [D]$ including the masked token. Also introduce a \textit{positional embedding} $p_i \in \mathbb{R}^K$ for each position $i \in [I]$.
    \item Add the context and positional embeddings and represent the sentence in matrix form:
    $$X := \left[ \beta_{x_1} + p_1, \dots,   \beta_{x_{i-1}} + p_{i-1}, \beta_{\texttt{[MASK]}} + p_i, \beta_{x_{i+1}} + p_{i+1}, \dots, \beta_{x_{I}} + p_{I} \right] \in \mathbb{R}^{K \times I}.$$
    \item Introduce \textit{query}, \textit{key} and \textit{value} matrices: $W^\mathcal{Q}, W^\mathcal{K}, W^\mathcal{V} \in \mathbb{R}^{K \times K}$.
    \item Calculate the attention-transformed matrix, where the softmax is applied column-wise:
    $$X' := W^\mathcal{V}X \cdot \textrm{softmax}\left(\frac{\left( W^\mathcal{Q} X \right)^\top W^\mathcal{K} X}{K}\right) \in \mathbb{R}^{K \times I}.$$
    \item Introduce a \textit{center embedding} $\delta_\ell \in \mathbb{R}^K$ for each token $\ell \in [D]$, which can be compactly represented as a matrix $\delta \in \mathbb{R}^{K \times D}$.
    \item Predict the masked token $x_i$ by applying a softmax function over the vocabulary. The probability distribution is given by
    $p(x_i \mid x_{-i}) \sim \textrm{Categorical}(\sigma(\delta^\top X_i'))$, where $\sigma$ and $X_i'$ represent the softmax operator and the $i$-th column of $X'$, respectively.
    \item Learn the parameters $\beta_\ell$'s, $p_i$'s, $\delta_\ell$'s, $W^\mathcal{Q}$, $W^\mathcal{K}$, and $W^\mathcal{V}$ by minimizing the sum of the categorical cross-entropy losses across all tokens in the data set (i.e., the MLM objective).
\end{enumerate}

\begin{remark}
    Note that this simplified architecture omits several components used in the actual BERT model, namely multi-head attention, multi-layer attention, dense layers, as well as residual connections and layer normalizations. Refer to \citet{devlin2019bert} for more details.
\end{remark}

\subsection{BERT as a generalization of CBOW}
\label{sec:bert-cbow}
We now present Proposition \ref{prop:bert-cbow}, which shows that the simplified BERT architecture in Section \ref{sec:bert} can be viewed as a generalization of the CBOW model. The proof is provided in Appendix \ref{app:pf-bert-cbow}.

% \begin{proposition}[BERT generalizes CBOW]
% \label{prop:bert-cbow}
%     The simplified BERT architecture in Section \ref{sec:bert} is a generalization of the CBOW model in Section \ref{sec:efe}, where all other words in the sentence serve as context words, i.e., $c_i := [I] - \{i\}$.
% \end{proposition}

As Proposition \ref{prop:bert-cbow} illustrates, CBOW is a special case of BERT and its MLM objective. Furthermore, as discussed in Section \ref{sec:efe}, CBOW can be viewed as a specific instance of EFE. Given these relationships, it is natural to extend EFE by incorporating the attention mechanism, similar to how BERT generalizes the CBOW model.

\begin{remark}
    It is easy to see that both CBOW and BERT can be modified to be unidirectional (considering only the left context of each word), e.g., by masking the attention weights.
\end{remark}

\subsection{EFA as a generalization of EFE}
\label{sec: efa-efe}
In Sections \ref{sec:bert} and \ref{sec:bert-cbow}, we demonstrated that BERT generalizes CBOW. This formulation addresses the three key limitations of CBOW. First, the attention mechanism allows the model to capture complex, non-linear relationships, overcoming the linearity of CBOW. Second, positional embeddings resolve the order invariance issue by explicitly incorporating word order. Lastly, by considering all words in the sentence as context, BERT eliminates the need for a fixed window size, making context definition more data-driven.

Inspired by BERT’s success in addressing the limitations of CBOW, we now introduce EFA, an extension of EFE that incorporates the attention mechanism. To concretize our discussion, we will revisit Examples \ref{ex:gauss} and \ref{ex:ratings} to illustrate how the attention-based approach can potentially improve the modeling of both Gaussian observations and movie ratings\footnote{Example \ref{ex:baskets} is simply CBOW applied to market basket data, and its EFA version resembles the architecture in Section \ref{sec:bert}.}.

\subsubsection{EFA for Gaussian observations}
\label{sec:efa-gauss-obs}
Recall that in Example \ref{ex:gauss}, we model each observation as $x_{i=(n,t)} \mid x_{c_i} \sim \mathcal{N}(\eta_i(x_{c_i}), \sigma^2)$, where $c_i := c_{(n,t)} = \{ (m,t) \mid m \in \textrm{KNN}(k, n)\}$ and $$\eta_i(x_{c_i}) := \rho_n^\top \sum_{m \in \textrm{KNN}(k, n)} \alpha_m x_{(m,t)}.$$

To establish a clearer connection with EFE, we impose the restriction that the center and context embeddings for each time series are identical, i.e., $\rho_n = \alpha_n$ for each $n \in [N]$. Moreover, each time series $n \in [N]$ is associated with an \textit{attribute} $\tau_n \in \mathbb{R}^\tau$. For instance, in the zebrafish neurons example described in \citet{rudolph2016exponential}, the spatial location of each neuron can be considered its attribute. 

Lastly, we assume that each embedding is a learned (non-linear) function of its attribute, i.e., $\rho_n = \alpha_n = g(\tau_n)$ for some $g: \mathbb{R}^\tau \rightarrow \mathbb{R}^K$. This formulation offers more flexibility, as it enables us to generate embeddings for time series that are not in the training data, such as neurons at new spatial locations. In the modified EFE model, we thus have
$$\eta_i(x_{c_i}) := (g(\tau_n))^\top \sum_{m \in \textrm{KNN}(k, n)} g(\tau_m) x_{(m,t)},$$
where $g$ (e.g., parameterized by a neural network) is learned from the training data.

We now present a simple EFA architecture that is designed for the same data. Suppose that we are interested in modeling $x_{i = (n,t)} \in \mathbb{R}$ conditional on the observations at time step $t$ for the other time series.

\begin{enumerate}[leftmargin=0.6cm]
\item Let \[
X := 
\left[
  \begin{array}{ccccccc}
    \vrule & & \vrule & \vrule & \vrule & & \vrule \\
    g(\tau_1) & \ldots & g(\tau_{n-1}) & g(\tau_n) & g(\tau_{n+1}) & \ldots & g(\tau_N) \\
    \vrule & &\vrule & \vrule & \vrule & & \vrule \\
    x_{(1,t)} & \ldots & x_{(n-1,t)} & 0 & x_{(n+1,t)} & \ldots & x_{(N,t)}
  \end{array}
\right] \in \mathbb{R}^{(K+1) \times N},
\]
where we stack the embedding of each time series with its observation at time $t$. As we are interested in predicting $x_{i = (n,t)}$, we mask it by replacing the value with $0$.
\item Introduce \textit{query}, \textit{key} and \textit{value} matrices: $W^\mathcal{Q}, W^\mathcal{K}, W^\mathcal{V} \in \mathbb{R}^{(K+1) \times (K+1)}$.
\item Calculate the attention-transformed matrix:
    $$X' := W^\mathcal{V}X \cdot \left(\frac{\left( W^\mathcal{Q} X \right)^\top W^\mathcal{K} X}{K + 1}\right) \in \mathbb{R}^{(K+1) \times N}.$$
\item Predict the masked observation $x_{i=(n,t)}$ by applying a dense layer. The probability distribution is given by $x_{i=(n,t)} \mid x_{(-n,t)} \sim \mathcal{N}(Z^\top X_n', \sigma^2)$, where $Z \in \mathbb{R}^{K+1}$ and $X_n'$ represents the $n$-th column of $X'$.
\item Learn the parameters $g$, $W^\mathcal{Q}$, $W^\mathcal{K}$, $W^\mathcal{V}$, and $Z$ by maximizing the sum of the pseudo log-likelihood across all observations in the data set.
\end{enumerate}

\begin{remark}
\label{rmk:lin-sof}
    We use linear attention instead of softmax attention to establish a clearer connection with EFE. In practice, softmax attention can also be used.
\end{remark}

\begin{remark}
\label{rmk:comp-op}
    We can incorporate more complex non-linear operations into the EFA architecture, such as multi-head and multi-layer attention, dense layers, and residual connections. Additionally, we can increase the dimensionality of the $x_i$'s and introduce a learned embedding for the masked observation.
\end{remark}

\begin{remark}
    Note that no positional embeddings are used since the order in which the time series are observed does not matter in this case.
\end{remark}

We now present Proposition \ref{prop:gauss}, which demonstrates that the EFA architecture we just described is, in fact, a generalization of the modified EFE model. The proof is provided in Appendix \ref{app:pf-gauss}.

% \begin{proposition}[EFA generalizes EFE for Gaussian observations]
% \label{prop:gauss}
% The EFA architecture in Section \ref{sec:efa-gauss-obs} is a generalization of the modified EFE model, where all other time series serve as context, i.e., $k = N-1$. 
% \end{proposition}

To conclude, it is worth noting that this EFA formulation addresses some of the limitations of EFE by enabling the model to capture complex, non-linear relationships and eliminating the need to pre-define the notion of ``closeness'' and number of nearest neighbors $k$, which allows for a more data-driven approach to context definition.

\subsubsection{EFA for movie ratings} 
\label{sec:efa-movie}
Recall that in Example \ref{ex:ratings}, we model each observation as $$x_{i=(n,t)} - 1 \mid x_{c_i} \sim \textrm{Poisson}\left( \exp \left(  \rho_n^\top \hspace{1mm} \frac{\sum_{(m,t) \in c_i} \alpha_m x_{(m,t)}}{\left| c_i \right|} \right)\right),$$
where $c_i = c_{(n,t)} = \{ (m,t) \mid x_{(m,t)} \hspace{2mm} exists\}$. We now present a simple EFA architecture that models the same data. Let $|c_i| = J$, the rated movies (in chronological order) are $z_1, z_2, \dots, z_{J+1} \in [N]$, and $z_k = n$. Suppose that we are interersted in modeling the rating of the $k$-th movie rated by user $t$, i.e., $x_{i=(n,t)}$, given the ratings of other movies rated by the same user.
\begin{enumerate}[leftmargin=0.6cm]
\item Let \[
X := 
\left[
  \begin{array}{ccccccc}
    \vrule & & \vrule & \vrule & \vrule & & \vrule \\
    \beta_{z_1} & \ldots & \beta_{z_{k-1}} & \beta_n & \beta_{z_{k+1}} & \ldots & \beta_{z_{J+1}} \\
    \vrule & &\vrule & \vrule & \vrule & & \vrule \\
    \delta_{z_1} & \ldots & \delta_{z_{k-1}} & \delta_n & \delta_{z_{k+1}} & \ldots & \delta_{z_{J+1}} \\
    \vrule & &\vrule & \vrule & \vrule & & \vrule \\
    x_{(z_1,t)} & \ldots & x_{(z_{k-1},t)} & 0 & x_{(z_{k+1},t)} & \ldots & x_{(z_{J+1},t)}
  \end{array}
\right] \in \mathbb{R}^{(2K+1) \times (J+1)},
\]
where we stack the \textit{center} ($\beta$'s) and \textit{context} ($\delta$'s) \textit{embeddings} of each rated movie with its rating. As we are predicting $x_{i = (n,t)}$, we mask it by replacing the value with $0$.
\item Introduce a \textit{positional embedding} $p_i \in \mathbb{R}^{2K+1}$ for every position $i \in [J+1]$. Define $X^P := X + P \in \mathbb{R}^{(2K+1) \times (J+1)}$, where $P = [p_1, \dots, p_{J+1}] \in \mathbb{R}^{(2K+1) \times (J+1)}$.
\item Introduce \textit{query}, \textit{key} and \textit{value} matrices: $W^\mathcal{Q}, W^\mathcal{K}, W^\mathcal{V} \in \mathbb{R}^{(2K+1) \times (2K+1)}$.
\item Calculate the attention-transformed matrix:
    $$X' := W^\mathcal{V}X^P \cdot \left(\frac{\left( W^\mathcal{Q} X^P \right)^\top W^\mathcal{K} X^P}{J}\right) \in \mathbb{R}^{(2K+1) \times (J+1)}.$$
\item Predict the masked rating $x_{i=(n,t)}$. The probability distribution is given by $$x_{i=(n,t)} - 1 \mid x_{c_i} \sim \textrm{Poisson}\left( \exp \left(  Z^\top X_n' \right)\right),$$ where $Z \in \mathbb{R}^{2K+1}$ and $X_n'$ is the $n$-th column of $X'$.
\item Learn the parameters $\beta_i$'s, $\delta_i$'s, $p_i$'s, $W^\mathcal{Q}$, $W^\mathcal{K}$, $W^\mathcal{V}$, and $Z$ by maximizing the sum of the (pseudo) log-likelihood across all observations in the data set.
\end{enumerate}

\begin{remark}
Remarks \ref{rmk:lin-sof} and \ref{rmk:comp-op} also apply here. Moreover, we can impose the restriction that the center and context embeddings are identical to simplify the model.
\end{remark}

\begin{remark}
    Both EFA and EFE can easily be adapted to function unidirectionally (focusing only on movies rated earlier by the same user), e.g., by masking the attention weights.
\end{remark}

\begin{remark}
    Note that our EFA formulation directly extends to Bernoulli and Gaussian ratings as well.
\end{remark}

We now introduce Proposition \ref{prop:rating}, which shows that the EFA architecture is a generalization of the EFE model. The proof is provided in Appendix \ref{app:pf-prop-rating}.

% \begin{proposition}[EFA generalizes EFE for movie ratings]
% \label{prop:rating}
% The EFA architecture in Section \ref{sec:efa-movie} is a generalization of the EFE model.
% \end{proposition}

Note that this EFA formulation overcomes the inherent limitations of EFE by allowing the model to capture complex, non-linear relationships while also accounting for the order in which the movies are rated.

==> efe.tex <==
% !TeX root = ./main.tex

\section{Exponential Family Embeddings}
\label{sec:efe}
We begin by reviewing the standard \textit{Exponential Family Embeddings} (EFE) formulation in \citet{rudolph2016exponential}. Let our data be $x := x_{1:I}$, where $x_i \in \mathbb{R}^D$. For each $i \in [I]$, let $c_i \subseteq [I] - \{i\}$ denote its \textit{context}. The core idea of EFE is to model each data point based on its context. Concretely, $$x_i \mid x_{c_i} \sim \textrm{ExpFam}(\eta_i(x_{c_i}), t(x_i)),$$ where $\eta_i(x_{c_i})$ and $t(x_i)$ denote the natural parameter and sufficient statistic, respectively. \citet{rudolph2016exponential} uses the \textit{linear embedding}, defined as $$\eta_i(x_{c_i}) := f_i \left(\rho[i]^\top \sum_{j \in c_i} \alpha[j] x_j \right).$$ In this case, $f_i$ represents a predefined link function, while $\rho[i] \in \mathbb{R}^{K \times D}$ and $\alpha[i] \in \mathbb{R}^{K \times D}$ represent the center and context embeddings. These embeddings are learned via maximizing the sum of the pseudo log-likelihood across all data points, where the pseudo log-likelihood for a data point $x = x_{1:I}$ is given by $\sum_{i \in [I]} \log p(x_i \mid x_{c_i})$.

\begin{remark}
    If we restrict $c_i$ to contain only indices smaller than $i$, the pseudo log-likelihood becomes the full likelihood since $$\log p(x) := \sum_{i \in [I]} \log p(x_i \mid x_{1, 2, \dots, i-1}) = \sum_{i \in [I]} \log p(x_i \mid x_{c_i}).$$
\end{remark}

\noindent
\textbf{CBOW as an instance of EFE.} EFE draws inspiration from Continuous Bag of Words (CBOW) \citep{mikolov2013distributed}, a pre-transformer language model. The CBOW model aims to predict each word in a sentence based on its surrounding (context) words. This model can be interpreted as a specific instance of EFE, where 
(1) $D$ is the vocabulary size; (2) $x_i \in \{0,1\}^D$ is the one-hot encoding of the word in position $i$; (3) $c_i := \{ j \neq i, i - w \leq j \leq i + w, 1 \leq j \leq I\}$ ($w$ is the \textit{window size}); (4) the center and context embeddings are the same for each position, i.e., $\rho[i] = \rho$ and $\alpha[j] = \alpha$; $\eta_i := \eta_i(x_{c_i}) = \sigma(\rho^\top \alpha \sum_{j \in c_i} x_j) \in \mathbb{R}^D$, where $\sigma$ denotes the softmax operator; and (5) the distribution $p(x_i \mid x_{c_i})$ is $\textrm{Categorical}(\eta_i)$.

\noindent
\textbf{Examples of EFE.} To facilitate our discussions, we will now present three instances of EFE used to model various types of real-world data.

% \begin{example}[Gaussian observations; 
% \citet{rudolph2016exponential}]
% \label{ex:gauss}
%     We are given $N$ time series, each containing a single observation at each time step from $1$ to $T$. Denote the observation at time step $t$ for the $n$-th time series by $x_i = x_{(n,t)} \in \mathbb{R}$. We model the data as $x_{i=(n,t)} \mid x_{c_i} \sim \mathcal{N}(\eta_i(x_{c_i}), \sigma^2)$, where $c_i := c_{(n,t)} = \{ (m,t) \mid m \in \textrm{KNN}(k, n)\}$ and $$\eta_i(x_{c_i}) := \rho_n^\top \sum_{m \in \textrm{KNN}(k, n)} \alpha_m x_{(m,t)}.$$
%     Here, $KNN(k, n)$ refers to $k$ time series that are the ``closest" to $n$, where the notion of ``closeness" can be defined in any way we choose. Lastly, note that the center and context embeddings for each time series are the same across all time steps.
% \end{example}

% \begin{example}[Market baskets; \citet{chen2020studying}]
% \label{ex:baskets}
%     We are given $N$ market baskets, each containing a list of items purchased together in a single transaction. We can model these baskets using CBOW, where items and baskets are treated as words and sentences, respectively. When the ordering of items in each basket is unknown, we can treat all other items in the same basket as the context. The learned center and context embeddings of each item can then be used to identify complements and substitutes; see \citet{chen2020studying} for more details.
% \end{example}

% \begin{example}[Movie ratings; \citet{rudolph2016exponential}] 
% \label{ex:ratings}
% We are given $N$ movies and $T$ users. For each $n \in [N]$ and $t \in [T]$, let $x_{i=(n,t)} \in \{1,2,3\}$ be the rating given by user $t$ for movie $n$, if it exists. We define $c_i := c_{(n,t)} = \{ (m,t) \mid x_{(m,t)} \hspace{2mm} exists\}$ and model the data as
% $$x_{i=(n,t)} - 1 \mid x_{c_i} \sim \textrm{Poisson}\left( \exp \left(  \rho_n^\top \hspace{1mm} \frac{\sum_{(m,t) \in c_i} \alpha_m x_{(m,t)}}{\left| c_i \right|} \right)\right)$$
% or
% $$x_{i=(n,t)} \mid x_{c_i} \sim \textrm{Poisson}\left( 1 + \exp \left(  \rho_n^\top \hspace{1mm} \frac{\sum_{(m,t) \in c_i} \alpha_m x_{(m,t)}}{\left| c_i \right|} \right)\right).$$
% Note that the center and context embeddings for each movie are the same across all users. 
% \end{example}

==> intro-old.tex <==
% !TeX root = ./main.tex

\section{Introduction}
Word embeddings---such as Continuous Bag of Words (CBOW) \citep{mikolov2013distributed}, Global Vectors for Word Representation (GloVe) \citep{pennington2014glove}, and other approaches (e.g., \citet{bengio2006neural, mnih2013learning, levy2014neural, cotterell2017explaining, baer2018exponential})---have revolutionized natural language processing by introducing a way to represent words as high-dimensional dense vectors in continuous vector spaces. These embeddings are learned based on the idea that each \textit{center} word is governed by its surrounding (i.e., \textit{context}) words. \textit{Exponential Family Embeddings} (EFE) \citep{rudolph2016exponential} extends this concept, allowing for the modeling of diverse data types, such as time series, market baskets, and movie ratings.

EFE consists of three key components: the \textit{context}, the \textit{conditional exponential family}, and the \textit{embedding structure}. In the case of movie ratings, the context refers to other movies rated by the same user. Given this context, each movie's rating can be modeled as being Poisson-distributed, with the rate parameter depending on the ratings of the movies in the context. Finally, the embedding structure assigns shared center and context embeddings to each movie across users, capturing intrinsic properties such as genre or popularity.

Despite its versatility in modeling different types of data, EFE has some significant limitations. Like CBOW, which inspired its design, EFE \textit{assumes that the natural parameter is determined by a linear combination of latent vectors}. This limits the ability of EFE to capture complex, non-linear relationships within the data.

Furthermore, EFE \textit{does not account for the order of observations in the data}. For instance, in CBOW, the sequence of words in the context is assumed to have no influence on the conditional distribution of the center word given the context words. In the movie ratings example, the order in which a user rates movies is assumed not to affect the conditional distribution of the ratings given the context, though this may not always hold true.

Third, EFE \textit{lacks a flexible and data-driven way of defining the context}. In CBOW, the window size is assumed to be of a fixed size for every center word in any sentence, which may not always be realistic. Also, in the zebrafish neuron example from \citet{rudolph2016exponential}, defining the context involves both determining what ``closeness” means and selecting an appropriate value for the number of neighbors ($k$), which can be challenging.

\begin{figure}[t]
\centering
\includegraphics[width=16.25cm]{efa.png}
\caption{Examples of data that can be effectively modeled using exponential family attention (EFA): (\textit{left}) spatiotemporal data where each time series is associated with a specific (e.g., spatial) attribute; (\textit{center}) grocery basket data with a given order of purchased items; and (\textit{right}) movie rating data where the sequence in which users rate movies is known.}
\label{fig:efa}
\end{figure}

To address these limitations of EFE, we propose \textit{exponential family attention} (EFA), a generalization of EFE that incorporates the self-attention mechanism \citep{vaswani2017attention}. EFA is inspired by the Bidirectional Encoder Representations from Transformers (BERT) architecture and its masked language model objective \citep{devlin2019bert}, which can be viewed as a generalization of CBOW. 

EFA is capable of modeling a wide variety of real-world data just like EFE (see Figure \ref{fig:efa}). Moreover, it offers several additional advantages. First, the self-attention mechanism enables EFA to capture complex, non-linear relationships. Second, positional embeddings allow EFA to incorporate order information from the data. Lastly, the context is defined in a data-driven manner by considering all other elements as potential context, allowing EFA to capture more nuanced dependencies.



==> macros.tex <==
\usepackage[T1]{fontenc}
\usepackage{verbatim}
\usepackage{float}
\usepackage{bm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{breakurl}
\usepackage{multirow}
\usepackage{mathtools}
\RequirePackage{natbib}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}


\makeatletter


\bibpunct{(}{)}{;}{a}{,}{,}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% LyX specific LaTeX commands.
%% Because html converters don't know tabularnewline
\providecommand{\tabularnewline}{\\}
\floatstyle{ruled}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% User specified LaTeX commands.

\usepackage{amsthm}\usepackage{dsfont}\usepackage{array}\usepackage{mathrsfs}\usepackage{comment}

\usepackage{color}\usepackage{babel}
\newcommand{\mypara}[1]{\paragraph{#1.}}

\newcommand{\R}{\mathbb{R}}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\rd}{\mathrm{d}}
\newcommand{\diverge}{\textsc{d}}
\newcommand{\q}{\mathrm{q}}
\newcommand{\BF}{\textsc{bf}}
\newcommand{\gBF}{\mathrm{g}\textsc{bf}}
\newcommand{\semi}{\mathrm{sp}}


\DeclareRobustCommand{\vec}[1]{\bm{#1}}
\pdfstringdefDisableCommands{%
	\renewcommand{\vec}[1]{#1}%
}



\newcommand{\ab}{\mathbf{a}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
\newcommand{\bbf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bi}{\bmf{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bbm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}




\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\renewcommand{\H}{\mathbb{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}
\newcommand{\BW}{\text{BW}}


%----- calligraphic fonts -----%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}




%----- blackboard bold fonts-----%

\newcommand{\HH}{\mathbb{H}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\OOmega}{\mathbb{\Omega}}




%----- bold greek fonts -----%

\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bdelta}{\bm{\delta}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\bvarepsilon}{\bm{\varepsilon}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\bm{\vartheta}}
\newcommand{\bkappa}{\bm{\kappa}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bnu}{\bm{\nu}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\bvarpi}{\bm{\varpi}}
\newcommand{\brho}{\bm{\varrho}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\bvarsigma}{\bm{\varsigma}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bupsilon}{\bm{\upsilon}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bvarphi}{\bm{\varphi}}
\newcommand{\bchi}{\bm{\chi}}
\newcommand{\bpsi}{\bm{\psi}}
\newcommand{\bomega}{\bm{\omega}}

\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bTheta}{\bm{\Theta}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bUpsilon}{\bm{\Upsilon}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bOmega}{\bm{\Omega}}

%----- Some standard definitions -----%

\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}}}

\newcommand{\sgn}{\mathop{\mathrm{sgn}}}
\newcommand{\Tr}{\mathop{\mathrm{Tr}}}
\newcommand{\supp}{\mathop{\mathrm{supp}}}

\DeclareMathOperator{\var}{\text{Var}}
\DeclareMathOperator{\cor}{\rm Corr}
\DeclareMathOperator{\cov}{\rm Cov}
\DeclareMathOperator{\id}{\mathds{1}}  % Indicator
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}

\newcommand*{\zero}{{\bm 0}}
\newcommand*{\one}{{\bm 1}}

\newcommand{\diag}{{\rm diag}}
\newcommand{\Range}{{\rm Range}}

\newcommand{\di}{{\rm d}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%% Norms

\newcommand{\norm}[1]{||#1||}
\newcommand{\bignorm}[1]{\bigg|\bigg|#1\bigg|\bigg|}
\newcommand{\opnorm}[2]{| \! | \! | #1 | \! | \! |_{{#2}}}

%%%%% Dot product
\newcommand{\dotp}[2]{\langle{#1},{#2}\rangle}

%%%%  brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}


%%%%%%%%%  Other commands
\newcommand{\tp}{t_{\text{pert}}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\mcomment}[1]{\marginpar{\tiny{#1}}}
\newcommand{\fcomment}[1]{\footnote{\tiny{#1}}}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}


\makeatother



\theoremstyle{plain} \newtheorem{lemma}{\textbf{Lemma}}\newtheorem{theorem}{\textbf{Theorem}}\setcounter{theorem}{0}
\newtheorem{corollary}{\textbf{Corollary}} \newtheorem{assumption}{\textbf{Assumption}}
\newtheorem{example}{\textbf{Example}} \newtheorem{definition}{\textbf{Definition}}
\newtheorem{fact}{\textbf{Fact}} 
\newtheorem{condition}{Condition}
 \newtheorem{proposition}{\textbf{Proposition}}

\theoremstyle{definition}
\newtheorem{remark}{\textbf{Remark}}
\newtheorem{claim}{\textbf{Claim}}
\newtheorem{model}{\textbf{Model}}


\newcommand{\C}{\mathcal{C}} 
\renewcommand{\L}{\mathcal{L}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\sm}{\mathcal{P}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\diff}{\backslash}
\newcommand{\increaseto}{\nearrow}
\newcommand{\iid}{\stackrel{iid}{\sim}}
\newcommand{\ji}[1]{\{#1\}} 
\newcommand{\eqd}{\overset{d}{=}}
\newcommand\red[1]{{\color{red}{#1}}} 
\newcommand\blue[1]{{\color{blue}{#1}}} 
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\dto}{\stackrel{d}{\to}}
\newcommand{\W}{\textsc{w}}


 \newcommand{\ind}{\perp\!\!\!\!\perp} 

\newcommand{\tr}{\text{tr}}
\newcommand{\mle}{\text{MLE}}
\newcommand{\mmd}{\textsc{mmd}}
\newcommand{\ksd}{\textsc{ksd}}
\newcommand{\ATE}{\textsc{ATE}}
\newcommand{\CATE}{\textsc{CATE}}
\newcommand{\slab}{\text{slab}}
\newcommand{\pa}{\text{pa}}
\newcommand{\Do}{\text{do}}
\newcommand{\diam}{\text{diam}}
\renewcommand{\L}{\mathcal{L}}
\renewcommand{\P}{\mathbb{P}}
\renewcommand{\B}{\mathbb{B}}

\newcommand{\bbT}{\mathbb{T}}
\newcommand{\rmP}{\textrm{P}}
\newcommand{\rmQ}{\textrm{Q}}
\newcommand{\rmp}{\mathrm{p}}  % modified
\newcommand{\rmq}{\mathrm{q}} % modified
\newcommand{\rmm}{\textrm{m}}
\newcommand{\g}{\, | \,}
\newcommand{\mbx}{\mathbf{x}}
\newcommand{\s}{\, ; \,}
\newcommand{\KL}[2]{D_{\textsc{KL}}\left( #1 \parallel #2\right)}
\newcommand{\kl}[1]{\textsc{kl}\left(#1\right)}
\usepackage{cleveref}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{proposition}{Proposition}{Propositions}
\crefname{equation}{eq.}{eqs.}
\Crefname{equation}{Eq.}{Eqs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{algocf}{algorithm}{algorithms} 

%EB
\newcommand{\obs}{\textrm{o}}
\newcommand{\wto}{\xrightarrow{\mathrm{w}}}
\newcommand{\asto}{\overset{\text{a.s.}}{\to}}


%Tricks for saving space:
\usepackage{times}
\usepackage{mathptmx}
\usepackage{paralist}
\usepackage[compact]{titlesec}
\titlespacing{\section}{0pt}{0.5ex}{0.5ex}
\titlespacing{\subsection}{0pt}{0ex}{0ex}
\titlespacing{\subsubsection}{0pt}{0ex}{0ex}

